Average-Case Communication Complexity of Statistical Problems

We study statistical problems, such as planted clique, its variants, and sparse principal component analysis in the context of average-case communication complexity. Our motivation is to understand the statistical-computational trade-offs in streaming, sketching, and query-based models. Communication complexity is the main tool for proving lower bounds in these models, yet many prior results do not hold in an average-case setting. We provide a general reduction method that preserves the input distribution for problems involving a random graph or matrix with planted structure. Then, we derive two-party and multi-party communication lower bounds for detecting or finding planted cliques, bipartite cliques, and related problems. As a consequence, we obtain new bounds on the query complexity in the edge-probe, vector-matrix-vector, matrix-vector, linear sketching, and $\mathbb{F}_2$-sketching models. Many of these results are nearly tight, and we use our techniques to provide simple proofs of some known lower bounds for the edge-probe model.

==> semi-random.tex <==

The semi-random model was introduced by Blum and Spencer \cite{BLUM1995204}. There are two variants of semi-random model and in this section we consider the sandwich model \cite{743518}. In this model, there is an adversary which can remove arbitrary edges outside the planted clique. We describe our hypothesis testing problem as follows:
\begin{itemize}
    \item $H_0$: the adversary could choose any graph $G^*$ such that $G_{\min}\subseteq G^*\subseteq G_{\max}$, where $G_{\max}$ is a random graph drawn from $G(n, 1/2)$ and $G_{\min}$ is the empty graph.
    \item $H_1$: the adversary could choose any graph $G^*$ such that $G_{\min}\subseteq G^*\subseteq G_{\max}$, where $G_{\max}$ is a random graph drawn from $G(n, 1/2, k)$ and $G_{\min}$ is the graph containing only the planted clique.
\end{itemize}

Since the adversary only removes edge outside the planted clique, we have the following upper bound directly from theorem 1 of \cite{racz2019finding}.

\begin{theorem} For semi-random model, suppose $k\ge (2+\eps) \log n$ for some constant $\eps > 0$, there exists an algorithm which can distinguish $H_0$ and $H_1$ with high probability, using $\tilde{O}(n^2/k^2)$ edge queries.
\end{theorem}

And our techniques would give a lower bound to this problem.

\begin{theorem} For semi-random model, suppose $k\le \sqrt{n}$, $\tilde{\Omega}(n^2/k^2)$ ??? queries is required to distinguish $H_0$ and $H_1$ with high probability.
\end{theorem}
\begin{proof}
By \lemref{clique_partition}, we can partition $K_n$ into $\Theta(n^2/k^2)$ edge-disjoint cliques each with size $\Theta(k)$. Then we randomly color each edge in these cliques with red or blue with equal probability. Now we consider the two-player set disjointness problem with length $\Theta(n^2/k^2)$. Construct a graph $G$ as follows: for each bit, let $G$ contain the red edges in the clique if Alice has a 1 , and let $G$ contain the blue edges in the clique if Bob has a 1. So if there is at most a 1 at every position, $G$ can be viewed as an instance under $H_0$. And if there is a unique position such that both Alice and Bob have a 1, $G$ can be viewed as an instance under $H_1$. Thus we reduce the 2-player set disjointness problem to our semi-random planted clique, and therefore we get a $\tilde{\Omega}(n^2/k^2)$ lower bound for our semi-random planted clique problem.
\end{proof}
